Scalable 3D Panoptic Segmentation As Superpoint Graph Clustering

We introduce a highly efficient method for panoptic segmentation of large 3D point clouds by redefining this task as a scalable graph clustering problem. This approach can be trained using only local auxiliary tasks, thereby eliminating the resource-intensive instance-matching step during training. Moreover, our formulation can easily be adapted to the superpoint paradigm, further increasing its efficiency. This allows our model to process scenes with millions of points and thousands of objects in a single inference. Our method, called SuperCluster, achieves a new state-of-the-art panoptic segmentation performance for two indoor scanning datasets: $50.1$ PQ ($+7.8$) for S3DIS Area~5, and $58.7$ PQ ($+25.2$) for ScanNetV2. We also set the first state-of-the-art for two large-scale mobile mapping benchmarks: KITTI-360 and DALES. With only $209$k parameters, our model is over $30$ times smaller than the best-competing method and trains up to $15$ times faster. Our code and pretrained models are available at https://github.com/drprojects/superpoint_transformer.

==> 5_acknowledgements_short.tex <==
\paragraph*{Acknowledgements.} 
This work was funded by ENGIE Lab CRIGEN and carried out in the LASTIG research unit of Université Paris-Est.


==> _3_method_bk.tex <==



Our goal is to perform universal segmentation of a 3D point cloud $\cP$. In other words, we aim to predict for each point a class and, if appropriate, an object index.
Each point $p \in \cP$ is associated with its three-dimensional spatial position in $\bR^3$, a semantic label $k_p\in [1,K]$ with $K$ the total number of classes, and an object index $o_p$.
Points identified with a ``thing'' label (\eg chair, car) are given an index uniquely identifying the object to which they belong. Conversely, points with a ``stuff'' label (\eg road, wall) are assigned an index shared by all points in $\cP$ from the same class.

\subsection{Superpoint Graph Construction}
To efficiently analyze large 3D point clouds, we adopt a partitioning strategy: the points of $\cP$ are grouped into simple shapes called  superpoints. We can then connect adjacent superpoints to form a rich data structure, referred to as the \emph{superpoint graph} \cite{landrieu2018large}, which we augment with object-related variables.

\paragraph{Computing Superpoints.}
We partition the point cloud $\cP$ into a set of non-overlapping superpoints, denoted $\cS$, such that the union of all $s \in \cS$ equals $\cP$. The superpoints are group of adjacent 3D points designed to be geometrically \cite{guinard2017weakly} or semantically \cite{landrieu2019point,hui2021superpoint} homogeneous. Following the methodology proposed in \cite{landrieu2018large}, we define the superpoints as the constant components of a low-contour approximation of geometric and radiometric point features.

We associate to each superpoint $s$ a \emph{majority object} $\obj(s)$ defined as the most common object index within its point: $\obj(s) = \mode \{o_p \mid p  \in s \}$. 
As object transitions often  correlate with geometric or radiometric contrasts, we can expect that most superpoints have high object purity, \ie that their majority object accounts for most of their 3D points. 

We then use a superpoint-embedding network to assign to each superpoint $s\in\cS$ an embedding $e_s \in \bR^D$ of dimension $D$. We employ the SuperPoint Transformer (SPT) model \cite{robert2023efficient} for its efficiency and ability to leverage large spatial contexts. 

\paragraph{Superpoint Graphs.}
We can link adjacent superpoints based on a well-chosen notion of proximity, which depends on the sensor and the acquisition density, see \secref{sec:implem} for details. 
We denote by $\cG=(\cS,\cE)$ the resulting superpoint graph structure with $\cE \subset \cS\times \cS$.

We can compute an \emph{affinity} score $a_{s,t}$ to two adjacent superpoints $(s,t) \in \cE$. This score quantifies their mutual agreement on the object to which they belong:
\begin{align}
a_{s,t} = \frac12
\left(
\frac{\mid \obj(s) \cap t \mid}{\mid t\mid }
+
\frac{\mid \obj(t) \cap s \mid}{\mid s\mid }
\right)~,
\end{align}
where $\mid s \mid$ is the count of 3D points in a superpoint $s$. An affinity of $1$ implies that the superpoints belong to the same object, $0$ indicates they overlap different objects. Intermediate values denote varying degrees of overlap between the superpoints and their majority objects, see \figref{fig:affinity},

Assuming that we could perfectly predict the affinity scores $a$, we could cluster the graph $\cG$ by merging nodes with affinity. The resulting aggregation would constitute a high-quality segmentation, provided that the superpoints of $\cS$ have high object purity.

\begin{figure}[t]
    \centering
    \scriptsize
   \input{figures/affinity}
    \caption{{\bf True Affinity Score.} We compute for each pair of adjacent superpoint  $(s,t)$ an affinity score measuring the agreement of their majority instance $\obj(s)$ and $\obj(t)$.}
    \label{fig:affinity}
\end{figure}

\subsection{Model Supervision}

\begin{figure*}
    \centering
    \scriptsize
   \input{figures/pipeline}
    \caption{{\bf Superpoint Graph Clustering.} We illustrate the sequence of operations of  SuperCluster for a simplified scene with two objects: a chair and a sofa.
    \textbf{Sub-figure (a)} showcases the first stage of our process, where the point cloud is partitioned into connected \emph{superpoints} with simple geometric shapes.
    In \textbf{Sub-figure (b)}, we predict an affinity score for each pair of adjacent superpoints, indicating the likelihood that they belong to the same real-world object.
    In \textbf{Sub-figure (c)}, we also predict for each superpoint a semantic class distribution and an offset towards the centroid of the object they belong to.
    Finally, \textbf{Sub-figure (d)} leverages these predicted attributes to parameterize a graph clustering problem which merges superpoints with high-affinity, compatible class distribution, and consistent centroid prediction. The cluster resulting clusters define the instances of a universal 3D segmentation.
    }
    \label{fig:enter-label}
\end{figure*}
We formulate the universal 3D segmentation problem in a way that allows us to train our model with auxiliary tasks only: all prediction and losses only consider one or two superpoint at a time. This approach removes the need for actual segmentation during training, thereby bypassing the computationally expensive step of matching true instances with their predicted counterparts.

\paragraph{Predicting Affinity.}  
We first predict the affinity score between two adjacent superpoints $(s,t) \in \cE$. For this purpose, we train a function $\phi_{\text{affinity}}$ to map a symmetric combination of superpoint embedding vectors to a predicted affinity $\hat{a}{s,t}$:
\begin{align}
    \hat{a}_{s,t} =
    \sigmoid 
    \left(
    \phi_{\text{affinity}}
    \left(
        \left[
            \sfrac{1}{2} (e_s  + e_t)
            ,
            \mid e_s  - e_t \mid
        \right]
    \right)
    \right)~,
\end{align}
with $[\,,\,]$  the channelwise concatenation and $\mid \cdot \mid$ the termwise absolute value.
We can interpret $\hat{a}_{s,t}$ and ${a}_{s,t}$ as parameters of Bernoulli distributions and use their cross-entropy as supervision:
\begin{align}
\cL^\text{affinity}_{s,t}
=
{a}_{s,t} \log (\hat{a}_{s,t}) 
+
(1-{a}_{s,t}) \log (1-\hat{a}_{s,t})~.
\end{align}

\paragraph{Predicting Semantics.}
We predict for each superpoint $s$ a class distribution $\hat{k}_s = \softmax(\phi_{\text{class}}(e_s)) \in \bR^K$ with $\phi_{\text{class}}$ a learnable function. The distribution $\hat{k}_s$ is supervised by its cross-entropy against the true class of its majority object $\obj(s)$:
\begin{align}
    \cL^\text{class}_s &= \log \left( \hat{k}_s[k_{\obj(s)}]\right)~.
\end{align}
This loss is identical to the one used for superpoint-based semantic segmentation methods \cite{landrieu2018large,robert2023efficient}.

\paragraph{Predicting Centroid Offsets.}
We predict for each superpoint $s$ an offset $\hat{\delta}s = \phi_{\text{offset}}(e_s) \in \bR^3$ between the centroid of $s$ and the centroid of its majority object. This prediction is supervised using the $L_2$ norm:
\begin{align}
   \!\! \cL^\text{offset}_s &= \frac1\mu \Vert \centroid(s) + \hat{\delta}_s - \centroid(s) \Vert^2~,
\end{align}
where $\centroid$ of a superpoint of an object is the mean position of its associated 3D points, and $\mu$ a constant homogeneous to a surface.
For superpoints $s$ for which $k_{\obj(s)}$ is a ``stuff'' class and thus lack meaningful centroids, we set $\cL^\text{offset}_s=0$.

\paragraph{Loss Function.} We combine the three losses above into a single objective $\cL$:
\begin{align}
    \cL = 
    \sum_{s\in \cS}
      \frac{\mid s \mid}{\mid\cP\mid  } \left( \cL^\text{class}_s +  \cL^\text{offset}_s\right)
    +
    \sum_{(s,t) \in \cE} \frac{ \lambda \cL^\text{affinity}_{s,t}}{\mid\cE\mid}~,
\end{align}
with $\mid \cE \mid$ and $\mid \cP \mid$ the number of superpoint edges and 3D points, respectively. The hyper-parameter $\lambda$ determines the balance between classification and offset prediction. Note that these losses are simple classification and regression guided by the fixed association between superpoints and their majority object. The model can be trained without matching proposed instances and true objects and without predicting an actual 3D segmentation.

\subsection{Superpoint Graph Clustering}

We use the predicted node and edge attributes defined above to parameterize a graph clustering problem whose solution yields a universal segmentation of the point cloud $\cP$.

\paragraph{Parametrization.} 
We formulate a graph clustering problem which aims to merge adjacent superpoints with high predicted affinity and compatible classes and offset predictions. 
We first introduce a signal $x \in \bR^{(3+K) \times \cS}$ defined on the nodes of $\cG$. 
The value of $x_s$ of superpoint $s$ is composed of two parts, concatenated channelwise: the predicted centroid position of its majority object $x^\text{centroid}_s=\centroid(s) + \hat{\delta}_s$, and the predicted class score: $x^\text{class}_s=\hat{k}_s$. 
If the highest probability of $\hat{k}_s$ corresponds to a ``stuff'' class, we set $x^\text{centroid}_s=\centroid(s)$ as the centroid of stuff objects is not defined.

We also associate each pair of adjacent superpoint $(s,t) \in \cE$ with a weight representing the cost of assigning $s$ and $t$ to different clusters. This cost is inversely proportional to the predicted affinity: $w_{s,t}= 1/{(\hat{a}_{s,t} + \epsilon})$ with $\epsilon$ a small constant, taken as $0.1$ throughout this article.

We define the graph clustering problem as the approximation of the signal $x$ into constant components of $\cG$ such that the cuts between components have low weight:
\begin{align}
   \!\! y^\star =\!\! \argmin_{y \in  \bR^{(3+K) \times \cS}}
    \sum_{s \in \cS} d(x_s,y_s)
    + \!\!\!
    \sum_{(s,t) \in \cE} \!\!
   \eta w_{s,t} 
     [y_s \neq y_t]~,
     \label{eq:gmpp}
\end{align}
with $\eta$ a parameter determining the strength of the cut regularization, $[a \neq b]=0$ if $a=b$ and $1$ otherwise.
The distance function $d$ takes into account the dual spatial-semantic nature of the signal $x$:
\begin{align}
   \!\! d(x_s,y_s)\! =\!
    \Vert x^\text{centroid}_s-x^\text{centroid}_s\Vert^2
    +
    \KL(x^\text{class}_s,y^\text{class}_s)~,
\end{align}
with $y^\text{centroid}_s$ the $3$ first coordinate of $y_s$ and $y^\text{class}_s$ the $K$ last. The term $\KL$ denotes the Kullback-Leiber divergence between two distributions.
A solution $y^\star$ of \eqref{eq:gmpp} defines a clustering of the superpoint set $\cS$, whose clusters $\cC$ are the connected components of the graph $\cG$ that are constant with respect to $y^\star$. %
Each element of $\cC$ are clusters of superpoints, \ie a \emph{set of sets of 3D points}.

\paragraph{Solving the Problem.} The optimization problem formulated in \eqref{eq:gmpp} is extensively studied in the graph optimization literature. Referred to as the \emph{generalized minimal partition problem} \cite{landrieu2017cut}, this problem is related to the Potts models \cite{potts1952some} and image partitioning \cite{leclerc1989constructing,mumford1989optimal}. We can solve this problem efficiently with the parallel implementation of the $\ell_0$-cut pursuit algorithm \cite{raguet2019parallel}.

As the function minimized in \eqref{eq:gmpp} is neither differentiable nor continuous, we cannot easily backpropagate gradients back to $x$. However, We only need to solve this optimization problem to evaluate the model and never during training.

\paragraph{Converting to a Universal Segmentation.} 
We can derive semantic, instance and panoptic segmentations from the solution $\cC$ of the graph clustering problem.
\begin{itemize}
    \item {\bf Semantic segmentation:} we assign to each cluster $c$ the class corresponding the highest probability of $x^{\star,\text{class}}_s$ for any $s$ within $c$ (as they share the same value by design). We then associate this class to all the points belonging to the superpoints of cluster $c$.
    \item {\bf Instance segmentation:} We associate a unique object index to each clusters $c$ predicted as a ``thing'' class.
    \item {\bf Panoptic segmentation:} We also assign to  each cluster classified as ``stuff'' an index shared by all clusters predicted as the same class.
\end{itemize}








==> _3_method_bk2.tex <==



Our objective is to perform panoptic segmentation of a large 3D point cloud $\cP$ with potentially numerous and extensive objects.
For clarity, we first present our graph clustering formulation at the point level. We then explain how our approach can be supervised purely with local objectives, making its training particularly efficient. Finally, we detail how our method can be easily generalized to superpoints to further increase its scalability. 

\paragraph{Problem Statement.} Each point $p \in \cP$ is associated with  a semantic label $\cls(p)\in [1,C]$ with $C$ the total number of classes, and an object index $\obj(p) \in \mathbb{N}$.
Points identified with a ``thing'' label (\eg chair, car) are given an index uniquely identifying this object. Conversely, points with a ``stuff'' label (\eg road, wall) are assigned an index \emph{shared by all points with the same class} within $\cP$. Our goal is to recover the class and object index of all points in $\cP$.

\subsection{Panoptic Segmentation as Graph Clustering}

We propose viewing the panoptic segmentation task as grouping adjacent points with compatible class and object predictions.
We express this task as the approximation of a signal into constant components in a graph.
We connect the points of $\cP$ to their $K$ nearest neighbors and represent this adjacency structure with the graph $\cG=(\cP,\cE)$ where $\cE \subset \cP \times \cP$.

\paragraph{Object-Contrastive Graph Signal.}
The first step of our approach is to learn a vertex-valued signal $x$ such that adjacent points of the same object share the same value and points of distinct objects have different values. 
We construct this signal in two parts, concatenated channelwise: $x_p=[x^\text{class}_p,x^\text{contrast}_p]$. 

The first part $x^\text{class}_p\in [0,1]^C$ contains a probabilistic prediction on the semantic nature of the object $\obj(p)$. 
As the points of a given object share the same class and points with different classes cannot belong to the same object, this value makes a good candidate for an object-contrastive signal.
However, distinct objects of the same nature can be adjacent, such as stacked chairs or cars in traffic.
To address this issue, we also associate each point with a value $x^\text{contrast}_v\in \bR^D$, which we specifically train to take different values for adjacent but distinct objects. \secref{sec:supervision} details how these values are obtained and supervised.

\paragraph{Piecewise-Constant Approximation.}
In an ideal scenario, if we could predict a signal $x$ that is perfectly homogeneous within objects and contrasted at their border, we could  
compute its constant components to directly recover all objects.
In practice, $x$ is predicted by a learning model, which may lead to some variation within  objects or some borders being missed.
Therefore, we propose to compute a smooth approximation $y^\star$ of the learned signal $x$ and define the predicted object as the constant components of $y^\star$ instead.

To erase small variations and ambiguities in the predicted signal $x$, we penalize its reconstruction by the surface of its constant components. This regularizer corresponds to a well-known prior in 2D { \cite{leclerc1989constructing,mumford1989optimal} and 3D \cite{labatut2009robust} analysis. 
In practice, we use weighted cuts in the graph $\cG$ as a proxy for the surface of constant components \cite{guinard2017weakly,landrieu2019point}.
The edge weight $w_{p,q}>0$ represents the likelihood of two points $p$ and $q$ being in the same object. This leads us to define the low-cut piecewise-constant approximation of $x$ as the following optimization problem: 
\begin{align}
   y^\star = \!\!\!\!\argmin_{y \in  \bR^{(C+D) \times \cP}}
    \sum_{p \in \cP} d(x_p,y_p)
    + \!\!\!\!
    \sum_{(p,q) \in \cE} \!\!\!\!
   \lambda w_{p,q} [y_p \neq y_q]~,
     \label{eq:gmpp}
\end{align}
where $\lambda$ is a parameter determining the strength of the cut regularization, and $[a \neq b]=0$ if $a=b$ and $1$ otherwise.  The distance function $d$ takes into account the dual semantic-contrastive nature of the signal $x$:
\begin{align}
   \!\! d(x_p,y_q)\! =\!
   H(x^\text{class}_p,y^\text{class}_c)
   + \eta
    \Vert x^\text{contrast}_p-y^\text{contrast}_p\Vert^2
    ~,
     \label{eq:dist}
\end{align}
where $y^\text{class}_p$ is the first $C$ coordinate of $y_p$ and $y^\text{contrast}_p$ the last $D$, and $\eta>0$ a model parameter. The term $H(x,y)$ denotes the cross-entropy between two distributions: $H(x,y)=\sum_{c=1}^C y_c \log(x_c)$. 

\paragraph{Graph Clustering.} The solution $y^\star$ of \eqref{eq:gmpp} will assign identical values to adjacent points with compatible semantic predictions $x^\text{class}$ and similar contrastive embeddings $x^\text{contrast}$ while avoiding winding and intricate contours. Conversely, adjacent points with dissimilar values of $x$ will be placed in distinct constant components. Therefore, by defining our clustering $\cK$ of $\cP$ as the constant components of $y^\star$, we group adjacent points with compatible object information.

\paragraph{Converting to a Panoptic Segmentation.} 
We can derive a panoptic segmentation from the clusters $\cK$. 
We first assign to each cluster $k$ the class corresponding to the highest probability of $y^{\star,\text{class}}_p$ for any point $p$ in $k$
(all points within $k$ share the same value by construction).
We then associate a unique object index to each cluster $k$ predicted as a ``thing'' class. Likewise, we assign to each cluster classified as ``stuff'' an index shared by all clusters predicted as the same class. Finally, we associate to each point with the class and object index of the cluster to which they belong.

\paragraph{Optimization.}
The optimization problem expressed in \eqref{eq:gmpp} is widely explored within graph optimization literature.
Referred to as the \emph{generalized minimal partition problem} \cite{landrieu2017cut}, this problem is related to the Potts models \cite{potts1952some} and image partitioning techniques \cite{leclerc1989constructing,mumford1989optimal}. We 
propose to adapt the parallel $\ell_0$-cut pursuit algorithm \cite{raguet2019parallel} to our dual semantic-contrastive objective. The resulting algorithm is particularly scalable and can handle graphs with hundreds of millions of edges on a standard workstation. 

\paragraph{Model Tuning.} The functional minimized in \eqref{eq:gmpp} is noncontinuous and nondifferentiable almost everywhere. This makes it hard to compute gradients and perform backpropagation from $y^\star$ to $x$ or the parameters $\lambda$ and $\eta$. 
However, once our model is fully trained, we can tune the parameters $\lambda$ and $\eta$ to maximize target metrics on a held-out validation. As this step is particularly efficient, we can perform a grid search of over tens of pairs of values in a few minutes.

\subsection{Model Supervision}
\label{sec:supervision}
\begin{figure*}
    \centering
    \scriptsize
   \input{figures/pipeline}
    \caption{{\bf Superpoint Graph Clustering.} We illustrate the sequence of operations of  SuperCluster for a simplified scene with two objects: a chair and a sofa.
    \textbf{Sub-figure (a)} showcases the first stage of our process, where the point cloud is partitioned into connected \emph{superpoints} with simple geometric shapes.
    In \textbf{Sub-figure (b)}, we predict an affinity score for each pair of adjacent superpoints, indicating the likelihood that they belong to the same real-world object.
    In \textbf{Sub-figure (c)}, we also predict for each superpoint a semantic class distribution and an offset towards the centroid of the object they belong to.
    Finally, \textbf{Sub-figure (d)} leverages these predicted attributes to parameterize a graph clustering problem which merges superpoints with high-affinity, compatible class distribution, and consistent centroid prediction. The cluster resulting clusters define the instances of a universal 3D segmentation.
    }
    \label{fig:enter-label}
\end{figure*}

A major benefit of the approach presented in the previous section is that it can be entirely supervised with local auxiliary tasks: all losses only consider one or two points at a time.
This removes the need for computing actual segmentation during training, thereby bypassing the computationally expensive step of matching true instances with their predicted counterparts.

\paragraph{Predicting Semantics.}
We use a neural network to associate to each point $p$ of $\cP$ a feature vector $e_p$.
We then predict a class distribution $x^\text{class}_p = \softmax(\phi^{\text{class}}(e_p))$ with $\phi^{\text{class}}$ a Multi-Layer Perceptron (MLP). This distribution is supervised by its cross-entropy against the true class $\cls(p)$:
\begin{align}
\cL^\text{class}_{p}
=
H(x^\text{class}_p,\mathbf{1}(\cls(p)))~,
\label{eq:cls}
\end{align}
with $\mathbf{1}(c) \in \{0,1\}^C$ the one-hot embedding of class $c$.

\paragraph{Predicting Object Agreement.}  
We predict $x^\text{contrast}_p = \phi^\text{contrast}(e_p)$ within $\mathbb{S}_M$ the $M$-dimensional unit sphere using an MLP $\phi^\text{contrast}$ followed by $L_2$ normalization.
We use this value to predict the \emph{object agreement} $a_{p,q} \in[0,1]$ between two neighboring points $p$ and $q$ as:
\begin{align}
a_{p,q} =\exp
\left(
    -\frac1\rho \Vert x^\text{contrast}_p - x^\text{contrast}_q \Vert^2
\right)~,
\end{align}
where $\rho>0$ is a temperature parameter.
The \emph{true object agreement} $\hat{a}_{p,q}$ is assigned the value of $1$ if $\obj(p)=\obj(q)$ and $0$ otherwise.
We supervise $x^\text{contrast}_p$ with the cross-entropy between predicted and true object agreement: 
\begin{align}
\cL^\text{contrast}_{p,q}
=
H(\bernoulli(a_{p,q}),\bernoulli(\hat{a}_{p,q}))~,
\label{eq:affinity}
\end{align}
where $\bernoulli(a)$ denote the Bernoulli distribution parametrized by $a \in [0,1]$.

\paragraph{Loss Function.} We combine the two losses above into a single objective $\cL$:
\begin{align}
    \cL =     \frac1{\mid\cP\mid  }
    \sum_{p\in \cP}
\cL^\text{class}_p
    +
    \frac1{\mid\cE\mid  }\sum_{(p,q) \in \cE} {\cL^\text{contrast}_{p,q}}~,
\end{align}
with $\mid \cE \mid$ and $\mid \cP \mid$ the number of superpoint edges and 3D points, respectively.
\subsection{Extension to Superpoints}
In this section, we discuss the extension of our method to a superpoint-based approach for enhanced efficiency and scalability.

\paragraph{Motivation.}
We aim to design a panoptic segmentation method that can scale to large 3D point clouds. While the formulation presented in the previous section is advantageous, it still requires computing embeddings and predictions for each individual point, which can be memory-intensive and limits the volume of data that can be processed simultaneously.
We propose to group adjacent points with similar local geometry and color into \emph{superpoints}, and to only compute embeddings and predictions for superpoints and not individual points. By doing so, we drastically reduce the computational and memory requirements of our method, enabling it to handle larger 3D point clouds at once.


\paragraph{Computing Superpoints.}
We partition the point cloud $\cP$ into a set of non-overlapping superpoints $\cS$. %
Following the methodology proposed in \cite{landrieu2018large,guinard2017weakly}, we define the superpoints as the constant components of a low-contour approximation of geometric and radiometric point features.

Although the superpoints $\cS$ form a high-purity oversegmentation of $\cP$, some superpoints can span multiple objects. To account for this, we associate each superpoint $s$ with its \emph{majority-object} $\obj(s)$ defined as the most common object index within its points: $\obj(s) = \mode \{\obj(p) \mid p  \in s \}$. 
Likewise, we define $\cls(s)=\mode \{\cls(p) \mid p  \in s \}$. 

\paragraph{Adapting Graph Clustering.}
Our clustering step can be directly adapted by substituting the point set $\cP$ by the superpoints $\cS$, and defining the graph $\cG$ by connecting superpoints with adjacent points. All other steps are unchanged.

\paragraph{Superpoint Semantic Supervision.} 
We use a superpoint-embedding network to assign to each superpoint $s\in\cS$ an embedding $e_s$. We employ the SuperPoint Transformer model \cite{robert2023efficient} for its efficiency and ability to leverage large spatial contexts. 
We supervise the semantic superpoint prediction $x^\text{class}_s$ with \eqref{eq:cls} where we replace $\cls(p)$ by $\cls(s)$.

\paragraph{Superpoint Object Agreement Supervision.} 
While the true object agreement $\hat{a}_{p,q}$ between two points is binary, the agreement between superpoints spans a continuum. As illustrated in \figref{fig:affinity}, we quantify this agreement as: 
\begin{align}
\hat{a}_{s,t} = \frac12
\left(
\frac{\mid s \cap \obj(t) \mid}{\mid s\mid }
+
\frac{\mid t \cap \obj(s) \mid}{\mid t\mid }
\right)
~,
\end{align}
where 
$s \cap o \eqdef  \{ p \in s \mid \obj(p) =  o \}$ is the set of points of $s$ with the object index $o$, and $\mid s \mid$ is the count of 3D points in $s$. We can now supervise the predicted object agreement $a_{s,t}$ with \eqref{eq:affinity} unchanged.

\begin{figure}[t]
    \centering
    \scriptsize
   \input{figures/affinity}
    \caption{{\bf True Affinity Score.} We compute for each pair of adjacent superpoint $(s,t)$ an object agreement score $a_{s,t}$.}
    \label{fig:affinity}
\end{figure}



==> figures/nodegreenblue.tex <==
\fill[blue] (\xcoord,\ycoord) -- (\xcoord,\ycoord+\rsize/2) arc [start angle=90, delta angle=360, radius=\rsize/2] -- cycle;
\fill[green] (\xcoord,\ycoord) -- (\xcoord,\ycoord+\rsize/2) arc [start angle=90, delta angle=\rtheta, radius=\rsize/2] -- cycle;
\node[thick, circle, draw, minimum size=\rsize cm] (\nodename) at (\xcoord, \ycoord) {};


